On the Nature of the Unique H$\alpha$-Emitting T Dwarf 2MASS J12373919+6526148

We explore and discount the hypothesis that the strong, continual H$\alpha$-emitting T dwarf 2MASS J12373919+6526148 can be explained as a young, low gravity, very low mass brown dwarf. The source is already known to have a marginally-fainter absolute magnitude than similar T dwarfs with trigonometric parallax measurements, and has a tangential velocity consistent with old disk kinematics. Applying the technique of Burgasser, Burrows & Kirkpatrick on new near infrared spectroscopy for this source, estimates of its {\teff}, $\log{g}$ and metallicity ([M/H]) are obtained. 2M 1237+6526 has a {\teff} $\approx$ 800-850 K. If [M/H] is solar, $\log{g}$ is as high as $\sim$5.5 (cgs) and this source is older than 10 Gyr. We find a more plausible scenario to be a modestly subsolar metallicity ([M/H] = -0.2) and moderate $\log{g}$ $\sim$ 5.0, implying an age older than 2 Gyr and a mass greater than 0.035 M$_{\sun}$. The alternative explanation of the unique emission of this source, involving an interacting, close, double degenerate system, should be investigated further. Indeed, there is some evidence of a {\teff} $<$ 500 K companion to 2M 1237+6526 on the basis of a possible $Spitzer IRAC$ [3.6]--[4.5] color excess. This excess may, however, be caused by a subsolar metallicity.

==> readme <==
                                      September 27, 2006

This is the second revised (version 3) submission to ApJ (MS 65595),
entitled "On the Nature of the Unique H$\alpha$-Emitting T Dwarf 2MASS
J12373919+6526148"

The coauthors are James Liebert and Adam J. Burgasser 

James Liebert is the corresponding author at
Steward Observatory
University of Arizona
Tucson, AZ  85721
liebert@as.arizona.edu
(520) 621-4513 phone
(520) 621-1532 fax

The submitted files are: 
readme
ms.tex
tab1.tex
tab2.tex
f1.eps
f2a.eps
f2b.eps
f2c.eps
f2d.eps
f3.eps
f4.eps
f5.eps
(note that f5.eps is new) 

Page charges will be paid by:
Steward Observatory
Univ. of Arizona
Tucson, AZ  85721

Figures 1, 4 and 5 are to be color in the electronic journal only. 

----------

We again thank the referee, Gibor Basri, for a couple of further 
thoughts which caused us to submit a slightly-revised, hopefully 
final version of the paper.  

In Section 5, discussing Figure 5, we now note "..there is some spread
in $M_{[3.6]}$ along the envelope amongst objects in a given spectral
subclass, possibly due to classification uncertainties).

We have slightly modified Figure 5, adding "K" to the number 
for each model sequence temperature.  In the caption, we now say 
"Each spectral class is plotted as a black numeral if the subtype 
is exact, or as a red numeral is there is a 0.5 subtype to be 
added.  2M~1237+6526 is showed as the enlarged red "6" (for T6.5)."

We have removed the "throwaway sentence at the end about magnetic 
dynamos." 




